Fuzzy Difference-in-Discontinuities: Identification Theory and Application to the Affordable Care Act

This paper explores the use of a fuzzy regression discontinuity design where multiple treatments are applied at the threshold. The identification results show that, under the very strong assumption that the change in the probability of treatment at the cutoff is equal across treatments, a difference-in-discontinuities estimator identifies the treatment effect of interest. The point estimates of the treatment effect using a simple fuzzy difference-in-discontinuities design are biased if the change in the probability of a treatment applying at the cutoff differs across treatments. Modifications of the fuzzy difference-in-discontinuities approach that rely on milder assumptions are also proposed. Our results suggest caution is needed when applying before-and-after methods in the presence of fuzzy discontinuities. Using data from the National Health Interview Survey, we apply this new identification strategy to evaluate the causal effect of the Affordable Care Act (ACA) on older Americans' health care access and utilization.

==> acctocareFDfinDiscR1R2R42012NPARTD_r13.tex <==
High school dropout &       0.025         &       0.002         &       0.055         &       0.158         \\
                    &     (0.102)         &     (0.095)         &     (0.207)         &     (0.116)         \\
Observations        &        2541         &        2541         &         948         &        2540         \\


==> acctocareFDfinDiscR1R2R42012NPARTD_r14.tex <==
High school graduate&       0.066         &      -0.007         &       0.084         &       0.042         \\
                    &     (0.058)         &     (0.037)         &     (0.105)         &     (0.061)         \\
Observations        &        5514         &        5514         &        2182         &        5510         \\


==> acctocareFDfinDiscR1R2R42012NPARTD_r15.tex <==
At least some college&       0.018         &      -0.001         &       0.072         &       0.028         \\
                    &     (0.028)         &     (0.023)         &     (0.057)         &     (0.035)         \\
Observations        &       12291         &       12291         &        5166         &       12278         \\


==> acctocareFDfinDiscR1R2R42012NPARTD_r2.tex <==
High school dropout &      -0.014         &      -0.052         &      -0.105         &       0.304         \\
                    &     (0.211)         &     (0.164)         &     (0.333)         &     (0.205)         \\
Observations        &         964         &         964         &         405         &         964         \\


==> acctocareFDfinDiscR1R2R42012NPARTD_r3.tex <==
High school graduate&       0.095         &      -0.000         &       0.104         &       0.064         \\
                    &     (0.061)         &     (0.041)         &     (0.114)         &     (0.068)         \\
Observations        &        4074         &        4074         &        1614         &        4070         \\


==> acctocareFDfinDiscR1R2R42012NPARTD_r4.tex <==
At least some college&       0.007         &      -0.008         &       0.029         &       0.023         \\
                    &     (0.030)         &     (0.021)         &     (0.063)         &     (0.033)         \\
Observations        &        9721         &        9721         &        4104         &        9711         \\


==> acctocareFDfinDiscR1R2R42012NPARTD_r5.tex <==
High school dropout &       0.045         &       0.012         &       0.218         &       0.032         \\
                    &     (0.147)         &     (0.151)         &     (0.266)         &     (0.144)         \\
Observations        &        1577         &        1577         &         543         &        1576         \\


==> acctocareFDfinDiscR1R2R42012NPARTD_r6.tex <==
High school graduate&      -0.079         &      -0.035         &      -0.015         &      -0.076         \\
                    &     (0.145)         &     (0.092)         &     (0.189)         &     (0.098)         \\
Observations        &        1440         &        1440         &         568         &        1440         \\


==> acctocareFDfinDiscR1R2R42012NPARTD_r7.tex <==
At least some college&       0.088         &       0.035         &       0.283\sym{*}  &       0.056         \\
                    &     (0.078)         &     (0.090)         &     (0.151)         &     (0.117)         \\
Observations        &        2570         &        2570         &        1062         &        2567         \\


==> acctocareFDfinDiscR1R2R42012PARTD_r13.tex <==
High school dropout &       0.243         &       0.179         &      -0.279         &       0.223         \\
                    &     (0.282)         &     (0.250)         &     (0.805)         &     (0.315)         \\
Observations        &        3385         &        3385         &        1268         &        3382         \\


==> acctocareFDfinDiscR1R2R42012PARTD_r14.tex <==
High school graduate&       0.094         &       0.079         &       0.201         &       0.182         \\
                    &     (0.157)         &     (0.110)         &     (0.259)         &     (0.139)         \\
Observations        &        7023         &        7023         &        2828         &        7016         \\


==> acctocareFDfinDiscR1R2R42012PARTD_r15.tex <==
At least some college&       0.077         &       0.004         &       0.194         &       0.126         \\
                    &     (0.068)         &     (0.051)         &     (0.120)         &     (0.096)         \\
Observations        &       15122         &       15122         &        6366         &       15106         \\


==> acctocareFDfinDiscR1R2R42012PARTD_r2.tex <==
High school dropout &       0.428         &       0.272         &     -84.158         &       1.003         \\
                    &     (0.933)         &     (0.664)         & (16359.320)         &     (1.001)         \\
Observations        &        1366         &        1366         &         569         &        1365         \\


==> acctocareFDfinDiscR1R2R42012PARTD_r3.tex <==
High school graduate&       0.184         &       0.117         &       0.280         &       0.222         \\
                    &     (0.167)         &     (0.123)         &     (0.277)         &     (0.149)         \\
Observations        &        5230         &        5230         &        2095         &        5224         \\


==> acctocareFDfinDiscR1R2R42012PARTD_r4.tex <==
At least some college&       0.052         &      -0.016         &       0.152         &       0.103         \\
                    &     (0.075)         &     (0.053)         &     (0.126)         &     (0.097)         \\
Observations        &       12000         &       12000         &        5066         &       11988         \\


==> acctocareFDfinDiscR1R2R42012PARTD_r5.tex <==
High school dropout &       0.325         &       0.163         &       0.431         &      -0.006         \\
                    &     (0.298)         &     (0.299)         &     (0.704)         &     (0.313)         \\
Observations        &        2019         &        2019         &         699         &        2017         \\


==> acctocareFDfinDiscR1R2R42012PARTD_r6.tex <==
High school graduate&      -0.281         &      -0.080         &      -0.176         &      -0.051         \\
                    &     (0.295)         &     (0.183)         &     (0.557)         &     (0.292)         \\
Observations        &        1793         &        1793         &         733         &        1792         \\


==> acctocareFDfinDiscR1R2R42012PARTD_r7.tex <==
At least some college&       0.200         &       0.103         &       0.391         &       0.264         \\
                    &     (0.141)         &     (0.131)         &     (0.410)         &     (0.234)         \\
Observations        &        3122         &        3122         &        1300         &        3118         \\


==> acctocareFDfinDiscR1R2R42012altbw1_r2.tex <==
High school dropout &       0.159         &       0.053         &      -0.703         &       0.062         \\
                    &     (0.324)         &     (0.299)         &     (0.607)         &     (0.405)         \\
Observations        &         657         &         657         &         271         &         657         \\


==> acctocareFDfinDiscR1R2R42012altbw1_r3.tex <==
High school graduate&       0.049         &       0.107         &       0.083         &       0.103         \\
                    &     (0.092)         &     (0.070)         &     (0.124)         &     (0.065)         \\
Observations        &        2559         &        2559         &        1060         &        2556         \\


==> acctocareFDfinDiscR1R2R42012altbw1_r4.tex <==
At least some college&       0.046         &      -0.007         &       0.046         &      -0.009         \\
                    &     (0.035)         &     (0.026)         &     (0.063)         &     (0.045)         \\
Observations        &        6585         &        6585         &        2845         &        6584         \\


==> acctocareFDfinDiscR1R2R42012altbw1_r5.tex <==
High school dropout &       0.250         &       0.139         &       0.080         &      -0.127         \\
                    &     (0.203)         &     (0.222)         &     (0.414)         &     (0.174)         \\
Observations        &         994         &         994         &         365         &         994         \\


==> acctocareFDfinDiscR1R2R42012altbw1_r6.tex <==
High school graduate&      -0.251         &      -0.143         &       0.046         &       0.062         \\
                    &     (0.190)         &     (0.101)         &     (0.186)         &     (0.156)         \\
Observations        &         895         &         895         &         388         &         894         \\


==> acctocareFDfinDiscR1R2R42012altbw1_r7.tex <==
At least some college&       0.170\sym{*}  &       0.068         &       0.028         &      -0.029         \\
                    &     (0.093)         &     (0.085)         &     (0.195)         &     (0.165)         \\
Observations        &        1604         &        1604         &         678         &        1603         \\


==> acctocareFDfinDiscR1R2R42012sq_r2.tex <==
High school dropout &       0.092         &       0.242         &      -1.156         &       0.427         \\
                    &     (0.848)         &     (1.007)         &     (0.957)         &     (0.677)         \\
Observations        &        1366         &        1366         &         569         &        1365         \\


==> acctocareFDfinDiscR1R2R42012sq_r3.tex <==
High school graduate&       0.042         &       0.114         &      -0.051         &       0.088         \\
                    &     (0.092)         &     (0.074)         &     (0.123)         &     (0.053)         \\
Observations        &        5230         &        5230         &        2095         &        5224         \\


==> acctocareFDfinDiscR1R2R42012sq_r4.tex <==
At least some college&       0.058         &       0.009         &       0.098         &       0.040         \\
                    &     (0.038)         &     (0.026)         &     (0.064)         &     (0.051)         \\
Observations        &       12000         &       12000         &        5066         &       11988         \\


==> acctocareFDfinDiscR1R2R42012sq_r5.tex <==
High school dropout &       0.272         &       0.137         &      -0.395         &      -0.221         \\
                    &     (0.237)         &     (0.269)         &     (0.678)         &     (0.204)         \\
Observations        &        2019         &        2019         &         699         &        2017         \\


==> acctocareFDfinDiscR1R2R42012sq_r6.tex <==
High school graduate&      -0.132         &      -0.116         &       0.006         &       0.070         \\
                    &     (0.181)         &     (0.110)         &     (0.164)         &     (0.151)         \\
Observations        &        1793         &        1793         &         733         &        1792         \\


==> acctocareFDfinDiscR1R2R42012sq_r7.tex <==
At least some college&       0.216\sym{**} &       0.018         &       0.158         &      -0.085         \\
                    &     (0.107)         &     (0.099)         &     (0.211)         &     (0.173)         \\
Observations        &        3122         &        3122         &        1300         &        3118         \\


==> acctocareFDfinDiscR32012_r1.tex <==
Overall sample      &      -0.003         &       0.001         &       0.019         &      -0.021         \\
                    &     (0.031)         &     (0.022)         &     (0.060)         &     (0.034)         \\
Observations        &       14417         &       14417         &        5935         &       14404         \\


==> altacctocareFDfinDiscR1R2R42012NPARTD_r13.tex <==
High school dropout &       0.116         &       0.209         &       0.279\sym{**} &      -0.012         \\
                    &     (0.131)         &     (0.142)         &     (0.118)         &     (0.111)         \\
Observations        &        1157         &        1156         &        1156         &        1156         \\


==> altacctocareFDfinDiscR1R2R42012NPARTD_r14.tex <==
High school graduate&      -0.020         &       0.058         &      -0.004         &      -0.023         \\
                    &     (0.056)         &     (0.046)         &     (0.047)         &     (0.070)         \\
Observations        &        2543         &        2542         &        2542         &        2545         \\


==> altacctocareFDfinDiscR1R2R42012NPARTD_r15.tex <==
At least some college&       0.129\sym{***}&       0.051         &       0.030         &      -0.084\sym{*}  \\
                    &     (0.032)         &     (0.036)         &     (0.026)         &     (0.049)         \\
Observations        &        6067         &        6067         &        6067         &        6071         \\


==> altacctocareFDfinDiscR1R2R42012NPARTD_r2.tex <==
High school dropout &      -0.003         &       0.169         &       0.157         &       0.019         \\
                    &     (0.247)         &     (0.208)         &     (0.149)         &     (0.170)         \\
Observations        &         500         &         499         &         499         &         501         \\


==> altacctocareFDfinDiscR1R2R42012NPARTD_r3.tex <==
High school graduate&      -0.075         &       0.041         &      -0.022         &      -0.027         \\
                    &     (0.060)         &     (0.041)         &     (0.047)         &     (0.070)         \\
Observations        &        1888         &        1888         &        1888         &        1889         \\


==> altacctocareFDfinDiscR1R2R42012NPARTD_r4.tex <==
At least some college&       0.124\sym{***}&       0.055         &       0.016         &      -0.084\sym{*}  \\
                    &     (0.033)         &     (0.041)         &     (0.026)         &     (0.049)         \\
Observations        &        4864         &        4864         &        4864         &        4868         \\


==> altacctocareFDfinDiscR1R2R42012NPARTD_r5.tex <==
High school dropout &       0.160         &       0.325\sym{**} &       0.407\sym{**} &       0.016         \\
                    &     (0.259)         &     (0.160)         &     (0.176)         &     (0.123)         \\
Observations        &         657         &         657         &         657         &         655         \\


==> altacctocareFDfinDiscR1R2R42012NPARTD_r6.tex <==
High school graduate&       0.199         &       0.114         &       0.065         &       0.007         \\
                    &     (0.139)         &     (0.142)         &     (0.132)         &     (0.123)         \\
Observations        &         655         &         654         &         654         &         656         \\


==> altacctocareFDfinDiscR1R2R42012NPARTD_r7.tex <==
At least some college&       0.154         &      -0.003         &       0.128\sym{*}  &      -0.050         \\
                    &     (0.096)         &     (0.068)         &     (0.072)         &     (0.132)         \\
Observations        &        1203         &        1203         &        1203         &        1203         \\


==> altacctocareFDfinDiscR1R2R42012PARTD_r13.tex <==
High school dropout &       0.000         &       0.242         &       0.239         &       0.312         \\
                    &         (.)         &     (0.268)         &     (0.225)         &     (0.333)         \\
Observations        &         848         &         847         &         847         &        1601         \\
High school dropout &       0.000         &       0.242         &       0.239         &       0.312         \\
                    &         (.)         &     (0.268)         &     (0.225)         &     (0.333)         \\
Observations        &         848         &         847         &         847         &        1601         \\
High school dropout &       0.570         &       0.794\sym{*}  &       1.059\sym{**} &       0.312         \\
                    &     (0.620)         &     (0.476)         &     (0.502)         &     (0.333)         \\
Observations        &        1602         &        1601         &        1601         &        1601         \\


==> altacctocareFDfinDiscR1R2R42012PARTD_r14.tex <==
High school graduate&      -0.056         &       0.071         &       0.022         &      -0.142         \\
                    &     (0.111)         &     (0.076)         &     (0.085)         &     (0.164)         \\
Observations        &        1803         &        1803         &        1803         &        3359         \\
High school graduate&      -0.056         &       0.071         &       0.022         &      -0.142         \\
                    &     (0.111)         &     (0.076)         &     (0.085)         &     (0.164)         \\
Observations        &        1803         &        1803         &        1803         &        3359         \\
High school graduate&      -0.179         &       0.170         &       0.049         &      -0.142         \\
                    &     (0.172)         &     (0.124)         &     (0.132)         &     (0.164)         \\
Observations        &        3357         &        3356         &        3356         &        3359         \\


==> altacctocareFDfinDiscR1R2R42012PARTD_r15.tex <==
At least some college&       0.206\sym{***}&       0.000         &       0.000         &      -0.081         \\
                    &     (0.054)         &         (.)         &         (.)         &     (0.106)         \\
Observations        &        4116         &        4117         &        4117         &        7636         \\
At least some college&       0.206\sym{***}&       0.000         &       0.000         &      -0.081         \\
                    &     (0.054)         &         (.)         &         (.)         &     (0.106)         \\
Observations        &        4116         &        4117         &        4117         &        7636         \\
At least some college&       0.301\sym{***}&       0.166\sym{**} &       0.116\sym{**} &      -0.081         \\
                    &     (0.081)         &     (0.074)         &     (0.057)         &     (0.106)         \\
Observations        &        7632         &        7631         &        7631         &        7636         \\


==> altacctocareFDfinDiscR1R2R42012PARTD_r2.tex <==
High school dropout &      12.330         &      12.212         &      15.318         &       3.741         \\
                    &   (151.973)         &   (143.291)         &   (181.434)         &    (30.994)         \\
Observations        &         723         &         722         &         722         &         724         \\


==> altacctocareFDfinDiscR1R2R42012PARTD_r3.tex <==
High school graduate&      -0.232         &       0.165         &       0.020         &      -0.117         \\
                    &     (0.181)         &     (0.121)         &     (0.137)         &     (0.164)         \\
Observations        &        2495         &        2495         &        2495         &        2496         \\


==> altacctocareFDfinDiscR1R2R42012PARTD_r4.tex <==
At least some college&       0.310\sym{***}&       0.187\sym{**} &       0.080         &      -0.076         \\
                    &     (0.086)         &     (0.081)         &     (0.056)         &     (0.108)         \\
Observations        &        6119         &        6118         &        6118         &        6123         \\


==> altacctocareFDfinDiscR1R2R42012PARTD_r5.tex <==
High school dropout &       0.247         &       0.560\sym{*}  &       0.781\sym{*}  &       0.301         \\
                    &     (0.620)         &     (0.333)         &     (0.395)         &     (0.209)         \\
Observations        &         879         &         879         &         879         &         877         \\


==> altacctocareFDfinDiscR1R2R42012PARTD_r6.tex <==
High school graduate&       0.005         &       0.231         &       0.166         &      -0.280         \\
                    &     (0.376)         &     (0.349)         &     (0.307)         &     (0.368)         \\
Observations        &         862         &         861         &         861         &         863         \\


==> altacctocareFDfinDiscR1R2R42012PARTD_r7.tex <==
At least some college&       0.200         &      -0.035         &       0.336\sym{*}  &      -0.069         \\
                    &     (0.294)         &     (0.182)         &     (0.170)         &     (0.229)         \\
Observations        &        1513         &        1513         &        1513         &        1513         \\


==> altacctocareFDfinDiscR1R2R42012altbw1_r2.tex <==
High school dropout &      -0.460         &       0.376         &       0.300         &       0.305         \\
                    &     (0.557)         &     (0.423)         &     (0.341)         &     (0.439)         \\
Observations        &         344         &         343         &         343         &         345         \\


==> altacctocareFDfinDiscR1R2R42012altbw1_r3.tex <==
High school graduate&       0.027         &       0.100         &       0.047         &      -0.043         \\
                    &     (0.102)         &     (0.076)         &     (0.086)         &     (0.104)         \\
Observations        &        1250         &        1250         &        1250         &        1250         \\


==> altacctocareFDfinDiscR1R2R42012altbw1_r4.tex <==
At least some college&       0.106\sym{**} &       0.072\sym{*}  &       0.012         &      -0.083         \\
                    &     (0.040)         &     (0.041)         &     (0.029)         &     (0.052)         \\
Observations        &        3429         &        3429         &        3428         &        3430         \\


==> altacctocareFDfinDiscR1R2R42012altbw1_r5.tex <==
High school dropout &       0.219         &       0.258         &       0.349         &       0.111         \\
                    &     (0.431)         &     (0.186)         &     (0.211)         &     (0.155)         \\
Observations        &         458         &         458         &         458         &         457         \\


==> altacctocareFDfinDiscR1R2R42012altbw1_r6.tex <==
High school graduate&      -0.061         &       0.152         &       0.038         &       0.064         \\
                    &     (0.177)         &     (0.162)         &     (0.142)         &     (0.153)         \\
Observations        &         447         &         447         &         447         &         447         \\


==> altacctocareFDfinDiscR1R2R42012altbw1_r7.tex <==
At least some college&       0.264         &      -0.055         &      -0.026         &      -0.081         \\
                    &     (0.188)         &     (0.105)         &     (0.054)         &     (0.120)         \\
Observations        &         796         &         796         &         796         &         795         \\


==> altacctocareFDfinDiscR1R2R42012sq_r2.tex <==
High school dropout &      -0.300         &       0.045         &       0.096         &       0.092         \\
                    &     (0.541)         &     (0.420)         &     (0.274)         &     (0.312)         \\
Observations        &         723         &         722         &         722         &         724         \\


==> altacctocareFDfinDiscR1R2R42012sq_r3.tex <==
High school graduate&       0.046         &       0.116         &       0.038         &      -0.038         \\
                    &     (0.107)         &     (0.083)         &     (0.084)         &     (0.105)         \\
Observations        &        2495         &        2495         &        2495         &        2496         \\


==> altacctocareFDfinDiscR1R2R42012sq_r4.tex <==
At least some college&       0.153\sym{***}&       0.091\sym{**} &       0.038         &      -0.122\sym{**} \\
                    &     (0.041)         &     (0.042)         &     (0.028)         &     (0.056)         \\
Observations        &        6119         &        6118         &        6118         &        6123         \\


==> altacctocareFDfinDiscR1R2R42012sq_r5.tex <==
High school dropout &       0.194         &       0.291         &       0.357         &       0.121         \\
                    &     (0.536)         &     (0.226)         &     (0.250)         &     (0.202)         \\
Observations        &         879         &         879         &         879         &         877         \\


==> altacctocareFDfinDiscR1R2R42012sq_r6.tex <==
High school graduate&      -0.097         &       0.067         &      -0.056         &      -0.013         \\
                    &     (0.179)         &     (0.178)         &     (0.145)         &     (0.167)         \\
Observations        &         862         &         861         &         861         &         863         \\


==> altacctocareFDfinDiscR1R2R42012sq_r7.tex <==
At least some college&       0.119         &      -0.121         &      -0.099         &      -0.042         \\
                    &     (0.197)         &     (0.111)         &     (0.083)         &     (0.138)         \\
Observations        &        1513         &        1513         &        1513         &        1513         \\


==> altacctocareFDfinDiscR32012_r1.tex <==
Overall sample      &      -0.078\sym{**} &      -0.080\sym{**} &      -0.055\sym{**} &      -0.021         \\
                    &     (0.034)         &     (0.031)         &     (0.024)         &     (0.026)         \\
Observations        &        7196         &        7192         &        7193         &        7197         \\


==> empDfinDiscR1R2R42012_r1.tex <==
Overall sample      &      -0.030         &      -0.030         \\
                    &     (0.026)         &     (0.021)         \\
Observations        &       25159         &       25265         \\


==> empDfinDiscR1R2R42012_r10.tex <==
Hispanic (all)      &       0.023         &       0.053         \\
                    &     (0.060)         &     (0.051)         \\
Observations        &        2905         &        2915         \\


==> empDfinDiscR1R2R42012_r11.tex <==
Black or Hispanic (all)&      -0.008         &       0.027         \\
                    &     (0.047)         &     (0.037)         \\
Observations        &        4829         &        4850         \\


==> empDfinDiscR1R2R42012_r12.tex <==
Non-White (all)     &       0.041         &       0.048         \\
                    &     (0.038)         &     (0.032)         \\
Observations        &        6829         &        6878         \\


==> empDfinDiscR1R2R42012_r13.tex <==
High school dropout &      -0.016         &      -0.013         \\
                    &     (0.059)         &     (0.046)         \\
Observations        &        3336         &        3347         \\


==> empDfinDiscR1R2R42012_r14.tex <==
High school graduate&      -0.050         &      -0.093\sym{*}  \\
                    &     (0.049)         &     (0.050)         \\
Observations        &        6904         &        6933         \\


==> empDfinDiscR1R2R42012_r15.tex <==
At least some college&      -0.025         &      -0.005         \\
                    &     (0.035)         &     (0.027)         \\
Observations        &       14919         &       14985         \\


==> empDfinDiscR1R2R42012_r2.tex <==
High school dropout &      -0.028         &      -0.051         \\
                    &     (0.085)         &     (0.077)         \\
Observations        &        1444         &        1470         \\


==> empDfinDiscR1R2R42012_r3.tex <==
High school graduate&      -0.051         &      -0.129\sym{**} \\
                    &     (0.055)         &     (0.053)         \\
Observations        &        5147         &        5161         \\


==> empDfinDiscR1R2R42012_r4.tex <==
At least some college&      -0.061         &      -0.028         \\
                    &     (0.038)         &     (0.030)         \\
Observations        &       11739         &       11756         \\


==> empDfinDiscR1R2R42012_r5.tex <==
High school dropout &       0.014         &       0.012         \\
                    &     (0.075)         &     (0.063)         \\
Observations        &        2120         &        2141         \\


==> empDfinDiscR1R2R42012_r6.tex <==
High school graduate&      -0.039         &       0.013         \\
                    &     (0.105)         &     (0.093)         \\
Observations        &        1757         &        1772         \\


==> empDfinDiscR1R2R42012_r7.tex <==
At least some college&       0.111         &       0.100         \\
                    &     (0.072)         &     (0.066)         \\
Observations        &        2952         &        2965         \\


==> empDfinDiscR1R2R42012_r8.tex <==
White non-Hispanic (all)&      -0.055\sym{*}  &      -0.057\sym{**} \\
                    &     (0.031)         &     (0.026)         \\
Observations        &       18330         &       18387         \\


==> empDfinDiscR1R2R42012_r9.tex <==
Black non-Hispanic (all)&      -0.026         &       0.001         \\
                    &     (0.077)         &     (0.075)         \\
Observations        &        1924         &        1935         \\


==> empDfinDiscR1R2R42012altbw1_r2.tex <==
High school dropout &      -0.008         &      -0.045         \\
                    &     (0.115)         &     (0.102)         \\
Observations        &         666         &         674         \\


==> empDfinDiscR1R2R42012altbw1_r3.tex <==
High school graduate&      -0.032         &      -0.110         \\
                    &     (0.081)         &     (0.075)         \\
Observations        &        2461         &        2471         \\


==> empDfinDiscR1R2R42012altbw1_r4.tex <==
At least some college&      -0.038         &      -0.016         \\
                    &     (0.057)         &     (0.045)         \\
Observations        &        6260         &        6266         \\


==> empDfinDiscR1R2R42012altbw1_r5.tex <==
High school dropout &       0.022         &       0.029         \\
                    &     (0.103)         &     (0.083)         \\
Observations        &        1009         &        1014         \\


==> empDfinDiscR1R2R42012altbw1_r6.tex <==
High school graduate&      -0.015         &      -0.020         \\
                    &     (0.170)         &     (0.144)         \\
Observations        &         826         &         835         \\


==> empDfinDiscR1R2R42012altbw1_r7.tex <==
At least some college&       0.004         &       0.056         \\
                    &     (0.108)         &     (0.096)         \\
Observations        &        1465         &        1469         \\


==> empDfinDiscR1R2R42012sq_r2.tex <==
High school dropout &      -0.008         &      -0.079         \\
                    &     (0.125)         &     (0.111)         \\
Observations        &        1444         &        1470         \\


==> empDfinDiscR1R2R42012sq_r3.tex <==
High school graduate&      -0.009         &      -0.085         \\
                    &     (0.084)         &     (0.080)         \\
Observations        &        5147         &        5161         \\


==> empDfinDiscR1R2R42012sq_r4.tex <==
At least some college&      -0.052         &      -0.021         \\
                    &     (0.058)         &     (0.047)         \\
Observations        &       11739         &       11756         \\


==> empDfinDiscR1R2R42012sq_r5.tex <==
High school dropout &       0.035         &       0.028         \\
                    &     (0.108)         &     (0.086)         \\
Observations        &        2120         &        2141         \\


==> empDfinDiscR1R2R42012sq_r6.tex <==
High school graduate&      -0.047         &      -0.065         \\
                    &     (0.163)         &     (0.136)         \\
Observations        &        1757         &        1772         \\


==> empDfinDiscR1R2R42012sq_r7.tex <==
At least some college&       0.034         &       0.073         \\
                    &     (0.104)         &     (0.095)         \\
Observations        &        2952         &        2965         \\


==> inscovDfinDiscR1R2R42012NPARTDsq_r10.tex <==
Hispanic (all)      &      -0.008         \\
                    &     (0.102)         \\
Observations        &        2365         \\


==> inscovDfinDiscR1R2R42012NPARTDsq_r11.tex <==
Black or Hispanic (all)&      -0.033         \\
                    &     (0.072)         \\
Observations        &        3890         \\


==> inscovDfinDiscR1R2R42012NPARTDsq_r12.tex <==
Non-White (all)     &      -0.058         \\
                    &     (0.057)         \\
Observations        &        5515         \\


==> inscovDfinDiscR1R2R42012NPARTDsq_r13.tex <==
High school dropout &      -0.086         \\
                    &     (0.089)         \\
Observations        &        2503         \\


==> inscovDfinDiscR1R2R42012NPARTDsq_r14.tex <==
High school graduate&      -0.023         \\
                    &     (0.050)         \\
Observations        &        5420         \\


==> inscovDfinDiscR1R2R42012NPARTDsq_r15.tex <==
At least some college&       0.049         \\
                    &     (0.042)         \\
Observations        &       12147         \\


==> inscovDfinDiscR1R2R42012NPARTDsq_r2.tex <==
High school dropout &      -0.012         \\
                    &     (0.141)         \\
Observations        &        1036         \\


==> inscovDfinDiscR1R2R42012NPARTDsq_r3.tex <==
High school graduate&      -0.024         \\
                    &     (0.065)         \\
Observations        &        4002         \\


==> inscovDfinDiscR1R2R42012NPARTDsq_r4.tex <==
At least some college&       0.065         \\
                    &     (0.041)         \\
Observations        &        9517         \\


==> inscovDfinDiscR1R2R42012NPARTDsq_r5.tex <==
High school dropout &      -0.151         \\
                    &     (0.119)         \\
Observations        &        1658         \\


==> inscovDfinDiscR1R2R42012NPARTDsq_r6.tex <==
High school graduate&      -0.041         \\
                    &     (0.078)         \\
Observations        &        1418         \\


==> inscovDfinDiscR1R2R42012NPARTDsq_r7.tex <==
At least some college&      -0.005         \\
                    &     (0.091)         \\
Observations        &        2439         \\


==> inscovDfinDiscR1R2R42012NPARTDsq_r8.tex <==
White non-Hispanic (all)&       0.030         \\
                    &     (0.034)         \\
Observations        &       14555         \\


==> inscovDfinDiscR1R2R42012NPARTDsq_r9.tex <==
Black non-Hispanic (all)&      -0.060         \\
                    &     (0.093)         \\
Observations        &        1525         \\


==> inscovDfinDiscR1R2R42012PARTDsq_r10.tex <==
Hispanic (all)      &      -0.074         \\
                    &     (0.084)         \\
Observations        &        2891         \\


==> inscovDfinDiscR1R2R42012PARTDsq_r11.tex <==
Black or Hispanic (all)&       0.022         \\
                    &     (0.063)         \\
Observations        &        4811         \\


==> inscovDfinDiscR1R2R42012PARTDsq_r12.tex <==
Non-White (all)     &      -0.010         \\
                    &     (0.048)         \\
Observations        &        6830         \\


==> inscovDfinDiscR1R2R42012PARTDsq_r13.tex <==
High school dropout &       0.064         \\
                    &     (0.065)         \\
Observations        &        3325         \\
High school dropout &       0.064         \\
                    &     (0.065)         \\
Observations        &        3325         \\


==> inscovDfinDiscR1R2R42012PARTDsq_r14.tex <==
High school graduate&       0.043         \\
                    &     (0.057)         \\
Observations        &        6900         \\
High school graduate&       0.043         \\
                    &     (0.057)         \\
Observations        &        6900         \\


==> inscovDfinDiscR1R2R42012PARTDsq_r15.tex <==
At least some college&       0.028         \\
                    &     (0.034)         \\
Observations        &       14924         \\
At least some college&       0.028         \\
                    &     (0.034)         \\
Observations        &       14924         \\


==> inscovDfinDiscR1R2R42012PARTDsq_r2.tex <==
High school dropout &       0.274\sym{***}\\
                    &     (0.100)         \\
Observations        &        1451         \\


==> inscovDfinDiscR1R2R42012PARTDsq_r3.tex <==
High school graduate&       0.068         \\
                    &     (0.057)         \\
Observations        &        5136         \\


==> inscovDfinDiscR1R2R42012PARTDsq_r4.tex <==
At least some college&       0.024         \\
                    &     (0.035)         \\
Observations        &       11732         \\


==> inscovDfinDiscR1R2R42012PARTDsq_r5.tex <==
High school dropout &      -0.070         \\
                    &     (0.085)         \\
Observations        &        2111         \\


==> inscovDfinDiscR1R2R42012PARTDsq_r6.tex <==
High school graduate&      -0.032         \\
                    &     (0.096)         \\
Observations        &        1764         \\


==> inscovDfinDiscR1R2R42012PARTDsq_r7.tex <==
At least some college&       0.046         \\
                    &     (0.070)         \\
Observations        &        2955         \\


==> inscovDfinDiscR1R2R42012PARTDsq_r8.tex <==
White non-Hispanic (all)&       0.054\sym{*}  \\
                    &     (0.030)         \\
Observations        &       18319         \\


==> inscovDfinDiscR1R2R42012PARTDsq_r9.tex <==
Black non-Hispanic (all)&       0.176\sym{*}  \\
                    &     (0.099)         \\
Observations        &        1920         \\


==> inscovDfinDiscR1R2R42012_r1.tex <==
Overall sample      &       0.022         &      -0.020\sym{*}  &      -0.022         &      -0.001         &      -0.000         \\
                    &     (0.015)         &     (0.011)         &     (0.014)         &     (0.016)         &     (0.026)         \\
Observations        &       25149         &       25144         &       25265         &       25265         &       22829         \\


==> inscovDfinDiscR1R2R42012_r10.tex <==
Hispanic (all)      &      -0.029         &      -0.015         &      -0.155\sym{***}&      -0.029         &       0.114         \\
                    &     (0.068)         &     (0.039)         &     (0.050)         &     (0.066)         &     (0.077)         \\
Observations        &        2891         &        2890         &        2915         &        2915         &        2389         \\


==> inscovDfinDiscR1R2R42012_r11.tex <==
Black or Hispanic (all)&      -0.022         &      -0.026         &      -0.096\sym{**} &      -0.028         &       0.143\sym{**} \\
                    &     (0.044)         &     (0.027)         &     (0.037)         &     (0.045)         &     (0.061)         \\
Observations        &        4811         &        4810         &        4850         &        4850         &        4092         \\


==> inscovDfinDiscR1R2R42012_r12.tex <==
Non-White (all)     &      -0.032         &      -0.022         &      -0.034         &      -0.040         &       0.154\sym{***}\\
                    &     (0.035)         &     (0.020)         &     (0.028)         &     (0.037)         &     (0.051)         \\
Observations        &        6830         &        6829         &        6878         &        6878         &        5891         \\


==> inscovDfinDiscR1R2R42012_r13.tex <==
High school dropout &      -0.029         &      -0.054         &      -0.028         &      -0.038         &       0.100         \\
                    &     (0.049)         &     (0.051)         &     (0.064)         &     (0.050)         &     (0.068)         \\
Observations        &        3325         &        3324         &        3347         &        3347         &        2797         \\


==> inscovDfinDiscR1R2R42012_r14.tex <==
High school graduate&      -0.011         &      -0.045\sym{*}  &      -0.046         &      -0.042         &       0.056         \\
                    &     (0.032)         &     (0.025)         &     (0.029)         &     (0.035)         &     (0.052)         \\
Observations        &        6900         &        6898         &        6933         &        6933         &        6221         \\


==> inscovDfinDiscR1R2R42012_r15.tex <==
At least some college&       0.045\sym{**} &      -0.001         &      -0.005         &       0.025         &      -0.037         \\
                    &     (0.023)         &     (0.012)         &     (0.021)         &     (0.022)         &     (0.031)         \\
Observations        &       14924         &       14922         &       14985         &       14985         &       13811         \\


==> inscovDfinDiscR1R2R42012_r2.tex <==
High school dropout &       0.100         &      -0.015         &       0.206\sym{**} &       0.094         &       0.149         \\
                    &     (0.084)         &     (0.061)         &     (0.097)         &     (0.091)         &     (0.105)         \\
Observations        &        1451         &        1451         &        1470         &        1470         &        1304         \\


==> inscovDfinDiscR1R2R42012_r3.tex <==
High school graduate&      -0.009         &      -0.035         &      -0.051\sym{*}  &      -0.029         &      -0.040         \\
                    &     (0.034)         &     (0.025)         &     (0.028)         &     (0.036)         &     (0.053)         \\
Observations        &        5136         &        5134         &        5161         &        5161         &        4685         \\


==> inscovDfinDiscR1R2R42012_r4.tex <==
At least some college&       0.046\sym{*}  &      -0.009         &      -0.018         &       0.014         &      -0.055         \\
                    &     (0.024)         &     (0.011)         &     (0.020)         &     (0.022)         &     (0.034)         \\
Observations        &       11732         &       11730         &       11756         &       11756         &       10949         \\


==> inscovDfinDiscR1R2R42012_r5.tex <==
High school dropout &      -0.123\sym{*}  &      -0.038         &      -0.131\sym{*}  &      -0.130\sym{**} &       0.141         \\
                    &     (0.066)         &     (0.060)         &     (0.075)         &     (0.060)         &     (0.085)         \\
Observations        &        2111         &        2110         &        2141         &        2141         &        1723         \\


==> inscovDfinDiscR1R2R42012_r6.tex <==
High school graduate&      -0.033         &      -0.069         &      -0.025         &      -0.094         &       0.366\sym{***}\\
                    &     (0.059)         &     (0.046)         &     (0.075)         &     (0.063)         &     (0.094)         \\
Observations        &        1764         &        1764         &        1772         &        1772         &        1536         \\


==> inscovDfinDiscR1R2R42012_r7.tex <==
At least some college&       0.029         &       0.015         &       0.030         &       0.057         &       0.055         \\
                    &     (0.043)         &     (0.035)         &     (0.046)         &     (0.056)         &     (0.075)         \\
Observations        &        2955         &        2955         &        2965         &        2965         &        2632         \\


==> inscovDfinDiscR1R2R42012_r8.tex <==
White non-Hispanic (all)&       0.034\sym{*}  &      -0.018         &      -0.013         &       0.007         &      -0.038         \\
                    &     (0.018)         &     (0.012)         &     (0.015)         &     (0.018)         &     (0.027)         \\
Observations        &       18319         &       18315         &       18387         &       18387         &       16938         \\


==> inscovDfinDiscR1R2R42012_r9.tex <==
Black non-Hispanic (all)&      -0.021         &      -0.053         &      -0.002         &      -0.041         &       0.188\sym{*}  \\
                    &     (0.063)         &     (0.042)         &     (0.060)         &     (0.062)         &     (0.096)         \\
Observations        &        1920         &        1920         &        1935         &        1935         &        1703         \\


==> inscovDfinDiscR1R2R42012altbw1_r2.tex <==
High school dropout &       0.145         &      -0.008         &       0.262\sym{**} &       0.134         &       0.014         \\
                    &     (0.107)         &     (0.067)         &     (0.128)         &     (0.121)         &     (0.139)         \\
Observations        &         667         &         667         &         674         &         674         &         603         \\


==> inscovDfinDiscR1R2R42012altbw1_r3.tex <==
High school graduate&      -0.025         &      -0.042         &      -0.072         &      -0.072         &       0.013         \\
                    &     (0.054)         &     (0.037)         &     (0.046)         &     (0.058)         &     (0.087)         \\
Observations        &        2457         &        2455         &        2471         &        2471         &        2240         \\


==> inscovDfinDiscR1R2R42012altbw1_r4.tex <==
At least some college&       0.057\sym{*}  &      -0.041\sym{***}&      -0.036         &       0.050\sym{*}  &       0.009         \\
                    &     (0.032)         &     (0.012)         &     (0.026)         &     (0.028)         &     (0.049)         \\
Observations        &        6252         &        6251         &        6266         &        6266         &        5847         \\


==> inscovDfinDiscR1R2R42012altbw1_r5.tex <==
High school dropout &      -0.156         &      -0.099         &      -0.061         &      -0.154\sym{*}  &       0.298\sym{***}\\
                    &     (0.100)         &     (0.087)         &     (0.095)         &     (0.090)         &     (0.107)         \\
Observations        &        1006         &        1006         &        1014         &        1014         &         836         \\


==> inscovDfinDiscR1R2R42012altbw1_r6.tex <==
High school graduate&      -0.116         &      -0.132\sym{**} &      -0.131         &      -0.166\sym{*}  &       0.269\sym{**} \\
                    &     (0.083)         &     (0.058)         &     (0.087)         &     (0.083)         &     (0.130)         \\
Observations        &         831         &         831         &         835         &         835         &         727         \\


==> inscovDfinDiscR1R2R42012altbw1_r7.tex <==
At least some college&       0.032         &      -0.005         &      -0.012         &       0.036         &       0.145         \\
                    &     (0.060)         &     (0.054)         &     (0.060)         &     (0.088)         &     (0.088)         \\
Observations        &        1464         &        1464         &        1469         &        1469         &        1317         \\


==> inscovDfinDiscR1R2R42012sq_r2.tex <==
High school dropout &       0.107         &      -0.075         &       0.267\sym{**} &       0.147         &       0.054         \\
                    &     (0.111)         &     (0.060)         &     (0.131)         &     (0.123)         &     (0.139)         \\
Observations        &        1451         &        1451         &        1470         &        1470         &        1304         \\


==> inscovDfinDiscR1R2R42012sq_r3.tex <==
High school graduate&      -0.016         &      -0.044         &      -0.037         &      -0.058         &       0.026         \\
                    &     (0.056)         &     (0.041)         &     (0.047)         &     (0.061)         &     (0.090)         \\
Observations        &        5136         &        5134         &        5161         &        5161         &        4685         \\


==> inscovDfinDiscR1R2R42012sq_r4.tex <==
At least some college&       0.059\sym{*}  &      -0.058\sym{***}&      -0.046         &       0.048\sym{*}  &      -0.010         \\
                    &     (0.033)         &     (0.015)         &     (0.028)         &     (0.027)         &     (0.051)         \\
Observations        &       11732         &       11730         &       11756         &       11756         &       10949         \\


==> inscovDfinDiscR1R2R42012sq_r5.tex <==
High school dropout &      -0.145         &      -0.015         &      -0.110         &      -0.146         &       0.206\sym{*}  \\
                    &     (0.103)         &     (0.085)         &     (0.098)         &     (0.093)         &     (0.120)         \\
Observations        &        2111         &        2110         &        2141         &        2141         &        1723         \\


==> inscovDfinDiscR1R2R42012sq_r6.tex <==
High school graduate&      -0.077         &      -0.104         &      -0.067         &      -0.142         &       0.275\sym{**} \\
                    &     (0.088)         &     (0.066)         &     (0.091)         &     (0.091)         &     (0.137)         \\
Observations        &        1764         &        1764         &        1772         &        1772         &        1536         \\


==> inscovDfinDiscR1R2R42012sq_r7.tex <==
At least some college&       0.043         &       0.024         &       0.038         &       0.063         &       0.179\sym{*}  \\
                    &     (0.064)         &     (0.054)         &     (0.063)         &     (0.095)         &     (0.095)         \\
Observations        &        2955         &        2955         &        2965         &        2965         &        2632         \\


==> inscovmcaidDfinDiscR1R2R42012sq_r1.tex <==
Overall sample      &      -0.013         \\
                    &     (0.016)         \\
Observations        &       25135         \\


==> inscovmcaidDfinDiscR1R2R42012sq_r10.tex <==
Hispanic (all)      &       0.147\sym{*}  \\
                    &     (0.088)         \\
Observations        &        2889         \\


==> inscovmcaidDfinDiscR1R2R42012sq_r11.tex <==
Black or Hispanic (all)&       0.065         \\
                    &     (0.081)         \\
Observations        &        4806         \\


==> inscovmcaidDfinDiscR1R2R42012sq_r12.tex <==
Non-White (all)     &      -0.002         \\
                    &     (0.053)         \\
Observations        &        6825         \\


==> inscovmcaidDfinDiscR1R2R42012sq_r13.tex <==
High school dropout &       0.043         \\
                    &     (0.084)         \\
Observations        &        3324         \\


==> inscovmcaidDfinDiscR1R2R42012sq_r14.tex <==
High school graduate&      -0.099\sym{***}\\
                    &     (0.028)         \\
Observations        &        6896         \\


==> inscovmcaidDfinDiscR1R2R42012sq_r15.tex <==
At least some college&       0.013         \\
                    &     (0.020)         \\
Observations        &       14915         \\


==> inscovmcaidDfinDiscR1R2R42012sq_r2.tex <==
High school dropout &      -0.058         \\
                    &     (0.121)         \\
Observations        &        1448         \\


==> inscovmcaidDfinDiscR1R2R42012sq_r3.tex <==
High school graduate&      -0.087\sym{***}\\
                    &     (0.031)         \\
Observations        &        5133         \\


==> inscovmcaidDfinDiscR1R2R42012sq_r4.tex <==
At least some college&       0.009         \\
                    &     (0.017)         \\
Observations        &       11729         \\


==> inscovmcaidDfinDiscR1R2R42012sq_r5.tex <==
High school dropout &       0.126         \\
                    &     (0.118)         \\
Observations        &        2108         \\


==> inscovmcaidDfinDiscR1R2R42012sq_r6.tex <==
High school graduate&      -0.125\sym{**} \\
                    &     (0.062)         \\
Observations        &        1763         \\


==> inscovmcaidDfinDiscR1R2R42012sq_r7.tex <==
At least some college&      -0.001         \\
                    &     (0.058)         \\
Observations        &        2954         \\


==> inscovmcaidDfinDiscR1R2R42012sq_r8.tex <==
White non-Hispanic (all)&      -0.021         \\
                    &     (0.015)         \\
Observations        &       18310         \\


==> inscovmcaidDfinDiscR1R2R42012sq_r9.tex <==
Black non-Hispanic (all)&      -0.103         \\
                    &     (0.139)         \\
Observations        &        1917         \\


==> inscovmedicaidDfinDiscR1R2R42012_r1.tex <==
Overall sample      &       0.031\sym{***}\\
                    &     (0.004)         \\
Observations        &       15220         \\


==> inscovmedicaidDfinDiscR1R2R42012_r10.tex <==
Hispanic (all)      &       0.040\sym{**} \\
                    &     (0.018)         \\
Observations        &        1950         \\


==> inscovmedicaidDfinDiscR1R2R42012_r11.tex <==
Black or Hispanic (all)&       0.049\sym{***}\\
                    &     (0.014)         \\
Observations        &        3154         \\


==> inscovmedicaidDfinDiscR1R2R42012_r12.tex <==
Non-White (all)     &       0.057\sym{***}\\
                    &     (0.010)         \\
Observations        &        4363         \\


==> inscovmedicaidDfinDiscR1R2R42012_r8.tex <==
White non-Hispanic (all)&       0.021\sym{***}\\
                    &     (0.005)         \\
Observations        &       10857         \\


==> inscovmedicaidDfinDiscR1R2R42012_r9.tex <==
Black non-Hispanic (all)&       0.065\sym{**} \\
                    &     (0.026)         \\
Observations        &        1204         \\

